SF3D: Stable Fast 3D Mesh Reconstruction with UV-unwrapping and Illumination Disentanglement

We present SF3D, a novel method for rapid and high-quality textured object mesh reconstruction from a single image in just 0.5 seconds. Unlike most existing approaches, SF3D is explicitly trained for mesh generation, incorporating a fast UV unwrapping technique that enables swift texture generation rather than relying on vertex colors. The method also learns to predict material parameters and normal maps to enhance the visual quality of the reconstructed 3D meshes. Furthermore, SF3D integrates a delighting step to effectively remove low-frequency illumination effects, ensuring that the reconstructed meshes can be easily used in novel illumination conditions. Experiments demonstrate the superior performance of SF3D over the existing techniques. Project page: https://stable-fast-3d.github.io

==> fig/gso-relighting.tex <==
\begin{figure*}[ht!]
    \centering
\resizebox{.95\linewidth}{!}{ %< auto-adjusts font size to fill line
\renewcommand{\arraystretch}{0.6}%
\setlength{\tabcolsep}{0pt}%
\begin{tabular}{%
    @{}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}@{\hskip 1cm}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}@{\hskip 1cm}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}%
    @{}%
}
GT & TripoSR & Ours & GT & TripoSR & Ours & GT & TripoSR & Ours \\[-0em]
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/gt0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/triposr0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/ours0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/gt0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/triposr0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/ours0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/gt0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/triposr0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Grandfather/ours0004.jpg} \\[-0.5cm]

\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/gt0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/triposr0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/ours0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/gt0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/triposr0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/ours0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/gt0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/triposr0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Cactus/ours0004.jpg} \\[-0.4cm]

\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/gt0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/triposr0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/ours0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/gt0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/triposr0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/ours0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/gt0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/triposr0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Asus/ours0004.jpg} \\[-0.3cm]

\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/gt0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/triposr0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/ours0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/gt0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/triposr0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/ours0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/gt0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/triposr0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Ogre/ours0004.jpg} \\[-0.5cm]

\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/gt0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/triposr0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/ours0001.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/gt0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/triposr0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/ours0002.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/gt0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/triposr0004.jpg} &
\includegraphics[width=3cm]{img/tripo-ours-gso/Pot/ours0004.jpg}
\end{tabular}
} %< \resizebox
\vspace{-2mm}
\titlecaptionof{figure}{Relighting on GSO}{Notice that our method removes the light more consistently from the input image. Hence, it reduces the light bake-in noticeable in the Ogre. Additionally, due to our normal mapping and vertex offset, our objects provide nicer surfaces for relighting. This is especially visible in the product box.}
    \label{fig:gso-mesh-relight}
\end{figure*}

==> fig/nvs_comparison.tex <==
\begin{figure}[ht!]
    \centering
\resizebox{.95\linewidth}{!}{ %< auto-adjusts font size to fill line
\renewcommand{\arraystretch}{0.6}%
\setlength{\tabcolsep}{0pt}%
\begin{tabular}{%
    @{}%
    l
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}%
    >{\centering\arraybackslash}m{3cm}%
    @{}%
}
\rotatebox[origin=c]{90}{GT} & 
\includegraphics[width=3cm]{img/nvs/sofa/gt/0001.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/gt/0002.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/gt/0003.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/gt/0004.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/gt/0005.jpg} \\[0cm]

\rotatebox[origin=c]{90}{TripoSR} & 
\includegraphics[width=3cm]{img/nvs/sofa/triposr/0001.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/triposr/0002.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/triposr/0003.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/triposr/0004.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/triposr/0005.jpg} \\[0cm]

\rotatebox[origin=c]{90}{SV3D} & 
\includegraphics[width=3cm]{img/nvs/sofa/sv3d/0001.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/sv3d/0002.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/sv3d/0003.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/sv3d/0004.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/sv3d/0005.jpg} \\[0cm]

\rotatebox[origin=c]{90}{Ours} & 
\includegraphics[width=3cm]{img/nvs/sofa/ours/0001.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/ours/0002.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/ours/0003.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/ours/0004.jpg} &
\includegraphics[width=3cm]{img/nvs/sofa/ours/0005.jpg} \\[0.2cm]

\rotatebox[origin=c]{90}{GT} & 
\includegraphics[width=3cm]{img/nvs/excavator/gt/0001.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/gt/0002.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/gt/0003.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/gt/0004.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/gt/0005.jpg} \\[0cm]

\rotatebox[origin=c]{90}{TripoSR} & 
\includegraphics[width=3cm]{img/nvs/excavator/triposr/0001.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/triposr/0002.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/triposr/0003.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/triposr/0004.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/triposr/0005.jpg} \\[0cm]

\rotatebox[origin=c]{90}{SV3D} & 
\includegraphics[width=3cm]{img/nvs/excavator/sv3d/0001.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/sv3d/0002.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/sv3d/0003.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/sv3d/0004.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/sv3d/0005.jpg} \\[0cm]

\rotatebox[origin=c]{90}{Ours} & 
\includegraphics[width=3cm]{img/nvs/excavator/ours/0001.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/ours/0002.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/ours/0003.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/ours/0004.jpg} &
\includegraphics[width=3cm]{img/nvs/excavator/ours/0005.jpg} \\[0cm]

\end{tabular}
} %< \resizebox
\vspace{-2mm}
\titlecaptionof{figure}{Novel View Synthesis}{Even compared to SV3D, a SOTA diffusion-based method that takes 20 minutes per asset, our method produces more detailed assets that follow the geometry well.}
    \label{fig:nvs_comparison}
\end{figure}

==> latexmkrc-off <==
#!/usr/bin/perl

## Put this (Perl) file in the root of your Overleaf project. It overrides the
## `pdflatex` compilation command to run GhostScript as a post-process which will
## compress non-JPEG images to JPEG in the output PDF file. The JPEG quality
## settings are set to high to minimize the loss of image quality. This should
## work well even for images that contain a lot of high-frequency noise.
## To disable, simply rename the file to something other than latexmkrc.
##
## Created by Iliyan Georgiev.

## Quality settings
$PDF_VERSION = 1.4;
$IMG_DOWNSAMPLE = 'true';
$IMG_DOWNSAMPLE_DPI = 600;
$IMG_DOWNSAMPLE_THRESHOLD = 1.0;
$IMG_COMPRESSION_QFACTOR = 0.15;  # lower is better (try 0.08 for higher quality)
$PASSTHROUGH_JPEGS = 'true';

## Don't modify these, they are specified by Overleaf
$GS_INPUT_FILE = '%B.pdf';
$GS_OUTPUT_FILE = '%B-embed.pdf';

## You can try setting below: -dNEWPDF=true
## This fails in the current GhostScript v9.55 on Overleaf 
$GS_COMMAND = "gs
   -sDEVICE=pdfwrite
   -sOutputFile=$GS_OUTPUT_FILE
   -dCompatibilityLevel=$PDF_VERSION
   -dPDFSETTINGS=/default
   -dFastWebView=true
   -dEmbedAllFonts=true
   -dSubsetFonts=true
   -dCompressFonts=true
   -dDetectDuplicateImages=true
   -dDoThumbnails=false
   -dAutoRotatePages=/None
   -dDownsampleColorImages=$IMG_DOWNSAMPLE
   -dColorImageDownsampleType=/Bicubic
   -dColorImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dColorImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleGrayImages=$IMG_DOWNSAMPLE
   -dGrayImageDownsampleType=/Bicubic
   -dGrayImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dGrayImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleMonoImages=$IMG_DOWNSAMPLE
   -dMonoImageDownsampleType=/Subsample
   -dMonoImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dMonoImageResolution=$IMG_DOWNSAMPLE_DPI
   -dConvertCMYKImagesToRGB=true
   -dColorImageFilter=/DCTEncode
   -dGrayImageFilter=/DCTEncode
   -dMonoImageFilter=/CCITTFaxEncode
   -dColorConversionStrategy=/LeaveColorUnchanged
   -dPassThroughJPEGImages=$PASSTHROUGH_JPEGS
   -dProcessColorModel=/DeviceRGB
   -dRenderIntent=1
   -dDefaultRenderingIntent=/Perceptual
   -dUseArtBox
   -dNEWPDF=false
   -dNOPAUSE
   -dBATCH
   -c \"<< /ColorACSImageDict << /VSamples [ 1 1 1 1 ] /HSamples [ 1 1 1 1 ] /QFactor $IMG_COMPRESSION_QFACTOR /Blend 1 /ColorTransform 1 >> >> setdistillerparams\"
   -f $GS_INPUT_FILE";

## Remove new-line characters from GhostScript command
$GS_COMMAND =~ s/\n//g;

## Set the pdflatex command to be used by Overleaf
$pdflatex = "pdflatex %O %S; $GS_COMMAND; mv %B-embed.pdf %B.pdf";

## For debugging
# print "$GS_COMMAND\n";
# print "$pdflatex\n";

